Testing $C_k$-freeness in bounded-arboricity graphs

We study the problem of testing $C_k$-freeness ($k$-cycle-freeness) for fixed constant $k > 3$ in graphs with bounded arboricity (but unbounded degrees). In particular, we are interested in one-sided error algorithms, so that they must detect a copy of $C_k$ with high constant probability when the graph is $\epsilon$-far from $C_k$-free. We next state our results for constant arboricity and constant $\epsilon$ with a focus on the dependence on the number of graph vertices, $n$. The query complexity of all our algorithms grows polynomially with $1/\epsilon$. (1) As opposed to the case of $k=3$, where the complexity of testing $C_3$-freeness grows with the arboricity of the graph but not with the size of the graph (Levi, ICALP 2021) this is no longer the case already for $k=4$. We show that $\Omega(n^{1/4})$ queries are necessary for testing $C_4$-freeness, and that $\widetilde{O}(n^{1/4})$ are sufficient. The same bounds hold for $C_5$. (2) For every fixed $k \geq 6$, any one-sided error algorithm for testing $C_k$-freeness must perform $\Omega(n^{1/3})$ queries. (3) For $k=6$ we give a testing algorithm whose query complexity is $\widetilde{O}(n^{1/2})$. (4) For any fixed $k$, the query complexity of testing $C_k$-freeness is upper bounded by ${O}(n^{1-1/\lfloor k/2\rfloor})$. Our $\Omega(n^{1/4})$ lower bound for testing $C_4$-freeness in constant arboricity graphs provides a negative answer to an open problem posed by (Goldreich, 2021).

==> C4-lb1-copy-before.tex <==


We start by proving a lower bound for constant-arboricity graphs.
\begin{theorem} \label{thm:C4-const-alpha-lb}
Testing $C_4$-freeness in constant-arboricity graphs requires $\Omega(n^{1/4})$ queries for constant $\epsilon$.
\end{theorem}
We note that Theorem~\ref{thm:C4-const-alpha-lb} holds for two-sided error algorithms and not only one-sided error ones. 
\commentt{DR: Give result with dependence on $\eps$?}

\begin{proof}
For any (sufficiently large) $n$ we shall define two bipartite graphs, $G_0$ and $G_1$, where both have constant arboricity. The graph $G_0$ is $C_4$-free and  the graph $G_1$ is $\Omega(1)$-far from being $C_4$ free.
Based on each $G_b$, $b\in \bitset$ we have a distribution, $\calD_b$, whose support consists of graphs isomorphic to $G_b$ (that differ only in vertex and edge labelings), and each distribution is uniform over its support.
\commentt{Do we think of $G_b$ as unlabeled as opposed to the graphs in the support of the distributions or is it also labeled? Or is $G_b$ a graph with specific labelings, i.e., one in the support? it is just a formality}
We shall show that for a sufficiently large constant $c$, an algorithm that performs less than $n^{1/4}/c$ queries, cannot distinguish with success probability at least $2/3$ between a graph selected according to $\calD_0$ and a graph selected according to $\calD_2$. The lower bound stated in the theorem follows.

We start by defining $G_0$. The vertices in $G_0$ are partitioned into three sets: $X_0,Y_0,Z_0$,  where $x_0 = y_0(y_0-1)/2$. We set $y_0$ to be the largest odd integer satisfying $x_0+2y_0 \leq n$ (the reason for the factor 2 will become clear shortly), and $z_0 = n-(x_0+y_0)$.
For each pair of vertices in $Y_0$ there is a unique vertex in $X_0$ that neighbors exactly these two vertices.
% Each vertex in $X_1$ has exactly two neighbors in $Y_1$, where any two vertices in $X_1$ share at most one neighbor in $Y_1$. Similarly, each vertex in $X_2$ has exactly two neighbors in $Y_2$, where any two vertices in $X_2$ share at most one neighbor in $Y_2$.
The vertices in $Z_0$ have no incident edges.
% Hence, all vertices in $Z_0$ have degree 0, all those in $X_0$ have degree 2, and all
% those in $Y_0 $ has degree $y_0 - 1$.
By construction, $G_0$ is $C_4$-free, and we have $y_0 = \Theta(n^{1/2})$, $z_0 = \Theta(y_0)=\Theta(n^{1/2})$,  and $x_0 = \Theta(n)$.

Turning to $G_1$, its vertices are also partitioned into three sets: $X_1,Y_1,Z_1$, of sizes $x_1$, $y_1$ and $z_1$, respectively, where $X_1$ is further partitioned into two equal-size sets $X_1^1$ and $X_1^2$, and $Y_1$ is partitioned into two equal-size sets $Y_1^1$ and $Y_1^2$ (so that $x_1$ and $y_1$ are both even).
Here $x_1/2 = (y_1/2)^2$ so that $x_1 = y_1^2/2$, and we set $y_1 = 2(y_0-1)$ and $z_1 = n- (x_1+y_1)$. For each pair of vertices, $u^1 \in Y_1^1$ and $u^2 \in Y_1^2$ there is one vertex in $X_1^1$ that neighbors exactly these two vertices, and one vertex in $X_1^2$ that neighbors them. The vertices in $Z_1$ have
no incident edges. By construction, since there are $x_1/2 = \Theta(n)$ edge-disjoint $C_4$s in $G_1$, it is $\Omega(1)$-far from being $C_4$-free.

Comparing the two graphs we observe that the vertices in
$Z_1$ have degree 0, which is the same as those in $Z_0$, The vertices in $X_1$ have degree 2, which is the same as those in $X_0$, and  the vertices in $Y_1$ have degree $y_1/2 = y_0-1$, which is the same as those in $Y_0$.
Comparing the sizes of the sets of vertices, since $y_1 = 2(y_0-1)$, we get that
$$x_1 = y_1^2/2 = (y_0-1)^2/2 = y_0(y_0-1)/2 - (y_0-1)/2 = x_0 - \Theta(n^{1/2})\;,$$
and
$$z_1 = n-(x_1+y_1) = n - (x_0 + (3/2)(y_0-1)) = z_0 - (y_0/2 - 3/2)) = \Theta(n^{1/2})$$
(recall that $x_0 + 2y_0 \leq n$). \commentt{DR: maybe explain a bit more}).
% Hence, $z_0 = O(n^{1/2})$, $y_0 = \theta(n^{1/2})$ and $x_0 = \Theta(n)$. Each vertex in $X_1$ has exactly two neighbors in $Y_1$, where any two vertices in $X_1$ share at most one neighbor in $Y_1$. Similarly, each vertex in $X_2$ has exactly two neighbors in $Y_2$, where any two vertices in $X_2$ share at most one neighbor in $Y_2$. The vertices in $Z_0$ an no incident edges. By construction, $G_0$ is $C_4$-free.

We next define two processes, $\calP_0$ and $\calP_1$, where $\calP_b$, for $b\in \bitset$ constructs ``on the fly'' a graph selected  according to $\calD_b$ while answering the queries of a testing algorithm. We shall show that unless one of several events occurs, the distributions induced on the sequences of queries and answers are identical. Let $q^t$ denote the $t$th query of the algorithm and $a^t$ the answer it gets, so that both are random variables. The query $q^t$ may depend on the \emph{query-answer history} $(q^1,a^1),\dots,(q^{t-1},a^{t-1})$ and possibly randomness of the algorithm. Both processes maintain a \emph{Knowledge graph}, which contains the vertices and edges that appear in these questions and answers, where $K^t=(V^t,E^t)$ is the knowledge graph after the $t$th query is answered. Let $X^t$, $Y^t$ and $Z^t$ denote the subsets of vertices with degree $2$, $y_0-1$ and $0$, respectively.
(In principle, the knowledge graph should also include information about the degrees of vertices and pairs of vertices that are known not to have edges between them, but, as we discuss below, this will be implicit from the graph.)
To determine $a^t$ given $q^t$,
the process $\calP_b$ simply considers all graphs in the support of $\calD_b$ that are consistent with $K^{t-1}$, and selects an answer with probability proportional to the number of such graphs that are also consistent with this answer.

We assume that before asking a query concerning a vertex $v$ that is not in the knowledge graph, the algorithm performs a degree query $q^t$ on $v$ (which in particular determines whether $v$ belongs to $X^t$, $Y^t$ or $Z^t$).
If the answer to this query is $2$, then the algorithm performs two neighbor queries to get $v$s two neighbors.
Also, if the algorithm gets new vertex $v$ as an answer to a neighbor query from a vertex
$u \in Y^{t-1}$, then it performs a neighbor query on $v$ so as to gets its second neighbor.
A lower bound of $T$ on the query complexity of the algorithm under theses restrictions translates into a lower bound of $\Omega(T)$ without these restrictions. Note that the algorithm need not ask any further degree queries, as their answers are determined by the knowledge graph (which is known to be isomorphic to a subgraph of $G_0$ or $G_1$). Also note that because for each degree-2 vertex that is introduced into the graph, the algorithm obtains both its neighbors, we may assume (without loss of generality) that the algorithm does not perform any vertex-pair queries (as their answers would always be negative).


We observe that for both processes, if the algorithm performs $o(n^{1/2})$ queries, then the probability that any answer to a degree query (on a new vertex) in not $2$, is $o(1)$ (since $|Y_b|+|Z_b| = O(n^{1/2})$ for both $b=0$ and $b=1$). Let's refer to this ``bad'' event as $E_1$.
% From this point on we condition on $E_1$ not occurring. That is, all new vertices belong to $X^t$.
In addition, by the second restriction on the algorithm (i.e., that each degree-2 vertex essentially ``arrives with both its neighbors''), we have that for any neighbor query $q^t$ on a vertex in $Y^{t-1}$, the process $\calP_b$ answers with a vertex (in $X^t$) whose label is uniformly selected among all $n-|V^{t-1}|$ ``free'' labels. That is, the distribution on these answers is identical under both processes.


% We shall also assume that once a new vertex of degree $2$ (i.e., that belongs to $X^t$) is introduced into the knowledge graph (either following a degree query or an answer to a neighbor query for a vertex $u \in Y^{t-1}$), both its neighbors (in $Y^t$) are determined and provided to the algorithm ``for free''. Clearly, a lower bound  under this assumption provides a lower bound that is at least as high without this assumption.
% This assumption implies that there are no edges between vertices in the knowledge graph other than those that already appear in it.
% Hence,


It remains to analyze the answers to neighbor queries for vertices $v$ in $X^{t-1}$.
% choice of  neighbors of a newly introduced vertex $v$ in $X^t$.
If $v$ is the answer to a neighbor query from a vertex $u \in Y^{t-1}$, then each of the processes needs to select a single (additional) neighbor. Conditioned on this neighbor not belonging to $V^{t-1}$, for both processes, its label is uniformly distributed among all $n-|V^{t-1}|$ ``free'' labels. The same is true if $v$ is introduced following a degree query and both its neighbors are determined not to belong to $V^{t-1}$. We denote the event that we get at least one neighbor that already belongs to the knowledge graph, by $E_2$. Observe that conditioned on $E_1$ and $E_2$ not occurring,  the distributions on query-answer histories induced by the two processes, are identical (since, conditioned on these events, every degree query is answered by $2$, and every neighbor query is answered by a uniformly selected new label).

It hence remains to upper bound the probability of the event $E_2$, under both processes, when the algorithm performs at most $n^{1/4}/c$ queries, for some sufficiently large constant $c$. Consider any prefix $(q^1,a^1),\dots,(q^{t-1},a^{t-1})$ of the query-answer history (where neither event $E_1$ or $E_2$ has yet occurred), and the corresponding knowledge graph $K^{t-1}$.
Suppose that $q^t$ is a degree query for a vertex $v$ (that does not belong to $V^{t-1}$, and such that the answer to this query is $2$). Consider first the process $\calP_0$. Since for each pair of vertices in $Y_0$ there is a single vertex in $X_0$ that neighbors them, and there are at most $2(t-1)$ vertices in $Y^{t-1}$, the probability (over the distribution induced by $\calP_0$) that at least one of the neighbors of $v$ belongs to $Y^{t-1}$ is upper bounded by
$$\frac{2(t-1)\cdot y_0}{{y_0\choose 2}} < \frac{4t}{y_0} = \frac{c' t}{n^{1/2}}$$
 for a constant $c'$ (since $y_0 = \Theta(n^{1/2})$). A similar (slightly lower) upper bound is obtained for $\calP_0$ when $v$ is the answer to a neighbor query from a vertex $u \in Y^{t-1}$ (since one of $v$ neighbors is already determined to be $u$).

Turning to $\calP_1$, we get a similar upper bound. Namely, for a new vertex $v$ (with degree 2), the probability that at least one of its neighbors belongs to $Y^{t-1}$ is upper bounded by
$$\frac{2(t-1)\cdot y_1}{(y_1/2)^2} = \frac{8(t-1)}{y_1} <\frac{4t}{y_0}= \frac{c' t}{n^{1/2}}\;,$$
 and a similar upper bound holds when $v$ is an answer to a neighbor query from $u\in Y^{t-1}$.
 (The reason we got the same final upper bound for both $\calP_0$ and $\calP_1$ despite the distributions being different is that in both cases we over-counted the number of possible pairs of neighbors that intersect $Y^{t-1}$ for a new degree-2 vertex.)
  Summing over $t=1,\dots,T= c'''n^{1/4}$, we get that the probability that $E_2$ occurs (for either processes) is a small constant, as required.
\end{proof}

\medskip
We now turn to a lower bound on non-constant arboricity graphs for one-sided error algorithms. We assume that $\alpha =O(n^{1/2})$ (recall that every graph with  arboricity greater than $n^{1/2}$ must contain $C_4$s). \commentt{DR: The lower bounds hold when $\alpha$ is known, and for the upper bounds we'll address the case of not knowing $\alpha$. Do we need to discuss the constant-factor gap between $n^{1/2}/c'$ and $n^{1/2}$?}  The lower bound holds for $\alpha = \Omega(\log n)$. Note that the lower bound of Theorem~\ref{thm:C4-const-alpha-lb} also holds for $\alpha = O(\log n)$ that is non-constant, since we can also add to the graphs in the lower-bound construction a subgraph with arboricity $\alpha$ that is $C_4$-free. \commentt{DR: need to ad reference}

\begin{theorem}\label{thm:C4-gen-alpha-lb}
Testing $C_4$-freeness with one-sided error in graphs with arboricity $c\log n < \alpha < n^{1/2}/c'$ for sufficiently constants $c$ and $c'$ requires $\Omega(n^{1/4}\alpha^{1/2})$ queries for constant $\epsilon$.
\end{theorem}


In order to prove Theorem~\ref{thm:C4-gen-alpha-lb}, we define
a distribution %$\calD$  
over $n$-vertex graphs for which the following holds. First, with high probability, a graph selected according to %$\calD$ 
this distribution is $\Omega(1)$-far from being $C_4$-free. Second, the number of queries necessary to observe a $C_4$ with sufficiently high constant probability when the queries are answered by graph selected according to 
the distribution %$\calD$ 
is $\Omega(n^{1/4}\alpha^{1/2})$. 
% We start by describing $\calD$.
We shall define the distribution in two steps. First we define a distribution $\calD$ over graphs with multiple (parallel) edges, and then we use it to define a distribution $\calD'$ over graphs without multiple edges. \commentt{DR: should we just use the term parallel edges? or is it Ok that we use both terms?}


The vertex set of each graph in the support of $\calD$ is partitioned into five parts: $X_1$, $X_2$, $Y_1$, $Y_2$, and $Z$, where $|X_1| = |X_2|=n/4$, $|Y_1| = |Y_2| = n^{1/2}\alpha/4$ and $|Z| = n/2- n^{1/2}\alpha/2$. (We assume for simplicity that $n$ is divisible by 4 and that $n^{1/2}$ is an integer -- the more general case can be handled similarly by rounding.)

There is a bipartite graph between $X_b$ and $Y_{b'}$ for $b,b' \in \{1,2\}$, where vertices in $X_b$ have degree $\alpha$, vertices in $Y_{b'}$ have degree $n^{1/2}$ and vertices in $Z$ have degree $0$. \commentt{Is it really exactly $\alpha$ and $n^{1/2}$?} Each graph in the support of $\calD$ is defined by 4 matchings, each between two tables, where there are overall 8 tables: $T_{X_b,b'}$ for $b,b' \in \{1,2\}$ and $T_{Y_{b'},b}$ for $b,b' \in \{1,2\}$. For each for $b,b' \in \{1,2\}$, there is a matching between $T_{X_b,b'}$ and $T_{Y_{b'},b}$. The tables $T_{X_b,b'}$ are of dimensions $|X_b|\times \alpha$, and the dimensions of the tables $T_{Y_{b'},b}$, are of dimensions $|Y_{b'}|\times n^{1/2}$.

Denoting the vertices in $X_b$ by $x_{b,1},\dots,x_{b,|X_b|}$ and the vertices in $Y_{b'}$ by $y_{b',1},\dots,y_{b',|Y_b'|}$,
if entry $(i,j)$ in the first table is matched to entry $(i',j')$ in the second table, then
$T_{X_b,b'}[i,j] = (i',j')$ and $T_{Y_{b'},b}[i',j'] = (i,j)$, where
this means that there is an edge between $x_{b,i}\in X$ and $y_{b',i'}\in Y$, where this edge is the $((b-1)\cdot\alpha+j$)th edge incident to $x_{b,i}$ and the $(b'-1)\cdot n^{1/2}+j'$th edge incident to $y_{b',i'}$.
The distribution $\calD$ is uniform over the graphs in its support.

We define the \emph{extra multiplicity} of a graph $G$ as the total number of edges in $G$, minus the number of distinct edges. Thus, if between two vertices there are $\ell$ parallel edges, then this pair of vertices contributes $\ell-1$ to the extra multiplicity.
The distribution $\calD'$ (over graphs without multiple edges), is simply defined by the following process.
A graph $G$ is selected according to $\calD$, and it determines a graph $G' = \tau(G)$ by removing all occurrences of multiple edges but one per pair of vertices with at least one edge between them. The labels of the edges are modified so that they maintain the order of the first occurrence of each edge. \commentt{DR: Add example?}
Let $\Sup(\calD)$ ($\Sup(\calD')$) denote the support of $\calD$ ($\calD'$). \commentt{DR: some of what appears here might go to the preliminaries} Thus $\tau$ is a many-to-one and onto function from $\Sup(\calD)$ to $\Sup(\calD')$.


\begin{claim}\label{clm:D-C4-far}
With probability at least $1-XX$, a graph selected according to $\calD'$ is $\Omega(1)$-far from being $C_4$-free.
\end{claim}

\commentt{DR: we might want to first introduce some smaller subclaims (maybe this should be a lemma and they will be claims)}

\begin{proof}
In order to prove the claim we first show that with probability at least $1-XX$ over the choice of a graph $G$ according to $\calD$, the graph $G$ contains at least $n\alpha/c$ \emph{edge-disjoint} $C_4$s (when counting multiple edges as distinct).
%  and it contains at most $n\alpha/(2c)$ multiple edges.
In addition we show that with probability at least $1-YY$ over the choice of a graph $G$ according to $\calD$, 
% it contains 
the extra multiplicity of $G$ (as defined above) is at most $n\alpha/(2c)$.
% multiple edges. 
The claim follows by a union bound.

% We start by establishing the second subclaim. We shall actually prove a stronger statement: with probability at least $1-YY$, no edge has multiplicity of more than 2
% for every vertex $x \in X_2\cup X_2$, the number of distinct neighbors of $x$ in $Y_b$ for $b\in \{1,2\}$ is at least $\alpha/2$ and an analogous statement holds for  $y \in Y_1\cup Y_2$. To verify this consider any $x_{b,i}\in X_b$ and the matching of its corresponding entries $T_{X_b}[i,j]$ for $j=1,\dots,\alpha$.

% We now turn to the first subclaim, while we condition on the ``good events'' of the first subclaim holding for every $x\in X_1$ and $y\in Y_1$.
Consider first selecting the edges between $X_1$ and $Y_1$, between $X_1$ and $Y_2$ and between $X_2$ and $Y_1$.
%For each edge $(x,y) \in X_1\times Y_1$, where there are $|X_1| \cdot \alpha = \Theta(n\alpha)$ such edges, let
For each $x\in X_1$, let $\Gamma_2(x)$ denote the multiset of its neighbors in $Y_2$ (that is, if there are $t$ edges between $x$ and $y'$, then $y'$ appears $t$ times in $\Gamma_2(x)$), and similarly define $\Gamma_2(y)$ for each $y \in Y_2$. By construction, $|\Gamma_2(x)| = \alpha$ and $|\Gamma_2(y)| = n^{1/2}$.

Before continuing with adding edges between $X_2$ and $Y_2$, we show that with probability at least $1-XX'$, there is no edge in $(X_1\times Y_2) \cup (X_2 \times Y_1)$ whose multiplicity is larger than four. To this end, consider any vertex $x_{1,i} \in X_1$ (the same argument applies to $x_{2,i}\in X_2$). For any choice of five entries in row $i$ of $T_{X_1,2}$, 
% quadruple of entries $T_{X_1}[i,j_1],T_{X_1}[i,j_2],T_{X_1}[i,j_3]$, 
the probability that all these entries are matched to five entries
in the same row $i'$ of  $T_{Y_2,1}$, for some $i'$, is upper bounded by $(1/|Y_2|)^4 = O(1/(n^2\alpha^4)$.
The probability that this event occurs for any choice of five entries in row $i$ is hence $O(\alpha/n^2)$, and the probability that this occurs for some $i$ is $O(\alpha/n) = o(1)$.
From this point on we condition on the event, denoted $E_1$, that every edge in $X_1\times Y_2 \cup X_2 \times Y_1$ has multiplicity at most four.

Let $(x,y)$ be any fixed edge in $X_1\times Y_1$, where there are $|X_1| \cdot \alpha = \Theta(n\alpha)$ such edges.
Next consider the selection of edges incident to vertices in $\Gamma_2(y)$. Namely, assume without loss of generality that $\Gamma_2(y) = \{x_{2,1},\dots,x_{2,n^{1/2}}\}$, and $\Gamma_2(x) = \{y_{2,1},\dots,y_{2,\alpha}\}$. We match the entries $T_{X_2,2}[i,j]$ for $i=1,\dots,n^{1/2}$ and $j=1,\dots,\alpha$ to entries of $T_{Y_2,2}$ according to lexicographic order.
We define $s=|\Gamma_2(y)|\cdot \alpha = n^{1/2}\cdot \alpha$ random variables $\chi_1,\dots,\chi_s$, where $\chi_\ell = 1$ if the $\ell$th entry according to the above order is matched to an entry $T_{Y_2,2}[i',j']$ where $i'\in [\alpha]$ (so that $y_{2,i'}\in \Gamma_2(x)$). Let $\chi = \sum_{\ell=1}^s \chi_\ell$.  Observe that the number of $C_4$ that the edge $(x,y)$ participates in and contain a pair of vertices $x' \in X_2$ and $y' \in Y_2$, is lower bounded by $\chi$, and conditioned on the event $E_1$, it is upper bounded by
$16\cdot \chi$. \commentt{DR: maybe need to elaborate a bit more.}
While these random variables are not independent, we can bound the probability that $\chi \notin [\alpha/2,2\alpha]$
by considering related, independent random variables, as explained next.

%Specifically, %for the lower bound of $\alpha/2$, 
Observe that for each $\ell \in [s]$ 
and for any $\beta \in \{0,1\}^{\ell-1}$,
$$\Pr[\chi_\ell=1 \,|\, \chi_1\dots,\chi_{\ell-1}=\beta] = 
       \frac{\alpha\cdot n^{1/2} - \sum_{r=1}^{\ell-1}\beta_i}{\alpha\cdot n - (\ell-1))}\;.$$
Therefore, for any $\beta \in \{0,1\}^{\ell-1}$ such that $\sum_{r=1}^{\ell-1}\beta_i < \alpha/2$, we have that 
$$\Pr[\chi_\ell=1 \,|\, \chi_1\dots,\chi_{\ell-1}=\beta] \geq 
           \frac{\alpha\cdot n^{1/2} - \alpha/2} {\alpha\cdot n } = \frac{1}{n^{1/2}}-\frac{1}{2n}\;,$$
and for any $\beta \in \{0,1\}^{\ell-1}$ 
$$\Pr[\chi_\ell=1 \,|\, \chi_1\dots,\chi_{\ell-1}=\beta] \leq 
    \frac{\alpha\cdot n^{1/2}}{\alpha\cdot n - \alpha\cdot n^{1/2}} = \frac{1}{n^{1/2}-1}\;.$$

We can hence obtain an upper bound on the probability that $\chi < \alpha/2$ by considering $s$ independent random variables $\chi'_1,\dots,\chi'_s$, where $\Pr[\chi'_\ell=1] = \frac{1}{n^{1/2}}-\frac{1}{2n}$ and applying the multiplicative Chernoff bound. We get that the probability that $\sum_{\ell=1}^s \chi'_\ell < \alpha/2$ is $\exp(-\Omega(\alpha))$, so that the same statement holds for $\chi$. For an upper bound on the probability that $\chi > 2 \alpha$, consider $s$ independent random variables $\chi''_2,\dots,\chi''_s$, where $\Pr[\chi''_\ell=1] = \frac{1}{n^{1/2}-1}$. Here too by applying the multiplicative Chernoff bound we get that the probability that $\sum_{\ell=1}^s \chi'_\ell > 2\alpha$ is $\exp(-\Omega(\alpha))$, and the same statement holds for $\chi$.

Since $\alpha = \Omega(\log n)$, by taking a union bound over all edges between $X_1$ and $Y_1$, we get that 
with probability at least $1-XX$, every edge $(x,y)\in X_1\times Y_1$ participates in at least $\alpha/2$ $C_4$s with a vertex in $X_2$ and a vertex in $Y_2$, and at most $32\alpha$ such $C_4$s. We can hence get a set of at least $\alpha\cdot |X_1|/64 = \Omega(\alpha n)$ edges-disjoint $C_4$s by applying a simple iterative algorithm for constructing such a set. \commentt{DR: explain more/better?}

Finally, we  bound the extra multiplicity obtained.
% number of multiple edges \commentt{DR: need a better term: it is the number of times that we get an edge that we got before}. 
The expected number of ``extra'' parallel edges is upper bounded by 
$(n/2)\cdot {\alpha\choose 2} \cdot 4/ n^{1/2} \leq \alpha^2 n^{1/2}$. \commentt{TO BE finalized after setting parameters more precisely or maybe just upper bounding $\alpha$}
\end{proof}
% setting of $\chi_1,\dots,\chi_{\ell-1} \in \{0,1\}^{\ell-1}$, 
%%


\comment{DR: modifying next claim so that uses new $\calD$ (no multiple edges from the start)}

\begin{claim}\label{clm:D-C4-lb}
Let $\calA$ be an algorithm  that performs less than $n^{1/4}\alpha^{1/2}/c$ queries for a sufficiently large constant $c$. The probability that $\calA$ detects a $C_4$ in a graph selected according to $\calD$
% $\calD'$, 
is at most $1/3$.
\end{claim}

\begin{proof}
Similarly to the proof of Theorem~\ref{thm:C4-const-alpha-lb}, consider a process $\calP$ that answers the query of a testing algorithm while constructing a graph from $\Sup(\calD)$ (the support of $\calD$) on the fly. Here too we define a knowledge graph $K^t$ following the query-answer history $(q^1,a^1),\dots,(q^t,a^t)$ and we require the algorithm to perform a degree query on each vertex $v$ that is not yet in the knowledge graph before performing any other query involving it. The algorithm also receives the subset to which the new vertex belongs (as this is not be implied by the degree of the vertex). Let $X_1^t$, $X_2^t$, $Y_1^t$, $Y_2^t$ and $Z^t$ denote the corresponding subsets in the knowledge graph $K^t$. %\commentt{DR: assume $\alpha < n^{1/2}$?}

The set of edges in $K^t$ is denoted by $E^t$, where for each $e\in E^t$ there are two associated labels, 
$\phi^t_X(e)$ for its endpoint in $X^t = X_1^t \cup X_2^t$, and $\phi^t_Y(e)$ for its endpoint in $Y^t = Y_1^t \cup Y_2^t$.
 We assume that a neighbor query $(x_{b,i},j)$ is answered by a pair $(y_{b',i'},j')$ where
$y_{b',i'}$ is the $j$th neighbor of $x_{b,i}$ and $x_{b,i}$ is the $j'$th neighbor of $y_{b',i'}$. Similarly, if a vertex-pair query $(x_{b,i},y_{b',i'})$ is answered positively, then the algorithm also gets the corresponding edge labels $\phi_X$ and $\phi_Y$ for this edge. The knowledge graph also includes a set $\overline{E}^t$ of non-edges (corresponding to negative answers to vertex-pair queries).

%%%%%%%%%%%
\iffalse
Recall that each graph $G' \in \Sup(\calD')$ may correspond to several graphs in $\Sup(\calD)$. Namely, to all graphs in $\tau^{-1}(G')$. Hence, the weight of $G'$ according to $\calD'$ is %the fraction of these graphs in the support of $\calD$. 
$|\tau^{-1}(G')|/|\Sup(\calD)|$.
Therefore, 
\fi
%%%%%%
Similarly to 
the proof of Theorem~\ref{thm:C4-const-alpha-lb}, in order to
determine $a^t$ given $q^t$,
the process $\calP$ considers all graphs  $G\in \Sup(\calD)$ 
that are consistent with $K^{t-1}$, 
%such that $\tau(G)$ is consistent with $K^{t-1}$.
It then selects an answer with probability proportional to the number of such graphs $G$ for which %$\tau(G)$ 
$G$ is also consistent with this answer. 
% This is equivalent to selecting a graph $G$ in the support of $\calD$ uniformly among all those whose corresponding graph $G'$ in the support of $\calD'$ is consistent with $K^t$, and answering according to $G'$.

Consider any knowledge graph $K^{t-1}$ for $t < n^{1/4}\alpha^{1/2}/c$. 
% so that $|X_1^{t-1}|$, $|X_2^{t-1}|$, $|Y_1^{t-1}|$, $|Y_2^{t-1}|$ $|E^{t-1}|$ and $|\overline{E}^{t-1}|$ are all smaller than $n^{1/4}\alpha^{1/2}/c$. 
We would like to bound the probability that either a neighbor query or a vertex-pair query adds to the knowledge graph an edge $(x,y)$ that creates a $C_4$ in the knowledge graph. We shall actually bound the probability that a neighbor query is answered with \emph{some} vertex that already belongs to the knowledge graph or a vertex-pair query is answered positively (even if this does not reveal a $C_4$).
We shall refer to such an answer as a \emph{collision}. \commentt{DR: better term?}

Let $\calG(K^{t-1})$ denote the subset of graphs  $G\in \Sup(\calD)$ such that %$\tau(G)$ 
$G$ is consistent with $K^{t-1}$. For a query $q^t$ (either a neighbor query or a pair query), let $\calG_c(K^{t-1},q^t)$ denote the subset of graphs  $G\in \calG(K^{t-1})$ for which the answer to $q^t$ according to %$\tau(G)$ 
$G$ results in a collision, and similarly define $\calG_{nc}(K^{t-1},q^t)$ for the case in which the answer is not a collision. % (henceforth, non-collision graphs).

\smallskip\noindent
\textsf{Subclaim}~
\emph{
Let $K^{t-1}$ be any knowledge graph where $t < n^{1/4}\alpha^{1/2}/c$, and let $q^t$ be a neighbor or pair query.
Then 
$$ \frac{|\calG_{nc}(K^{t-1},q^t)|}{|\calG_{c}(K^{t-1},q^t)|} = \Omega(n^{1/4}\alpha^{1/2}) \;.$$
}

\smallskip
\noindent
\textsf{Proof:}~
In order to prove the subclaim we define an auxiliary bipartite graph $\calB(K^{t-1},q^t)$. Each node in $\calB(K^{t-1},q^t)$ corresponds to a graph $G \in \calG(K^{t-1})$.
% \commentt{DR: or should we say that its corresponding graph $G'$ is consistent with $K^{t-1}$, and maybe instead of $G'$ we need a notation like $\tau(G)$}. 
Nodes on the left side correspond to graphs in $\calG_{c}(K^{t-1},q^t)$, and nodes on the right side to graphs in $\calG_{nc}(K^{t-1},q^t)$.
 There is an edge between two nodes corresponding to graphs $G_1$ and $G_2$, if $G_2$ can be obtained from $G_1$ by a certain ``swap'' modification (which will be explained precisely below). We shall show that the number of nodes on the left is smaller by a factor of $\Omega(n^{1/4}\alpha^{1/2})$ than the number of nodes on the left by appropriately lower bounding the degree of the former and upper bounding the degree of the latter.
 From this point on we use the shorthand notations $\calB$, $\calG$, $\calG_c$ and $\calG_{nc}$ for $\calB(K^{t-1},q^t)$, $\calG(K^{t-1})$, $\calG_c(K^{t-1},q^t)$ and $\calG_{nc}(K^{t-1},q^t)$, respectively.

% Consider first the case of a neighbor query $q^t = (x_{b,i},j)$ for $x_{b,i}\in X_b^{t-1}$, where $b\in \{1,2\}$.

%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
For the sake of the exposition, suppose first for simplicity that graphs in $\calG$ have no parallel edges, so that $\tau(G)=G$ for every $G\in \calG$.  \commentt{DR: maybe say somewhere that if on parallel edges were created in $\calD$, then the entire argument would have been much simpler and explain where the difficulty is?}
\fi
%%%%%%%%%%%%%%%%%%%%%
For a graph $G\in \calG$ and an edge $e$ in $G$ we shall use the notation $\phi^{G}_X(e)$
and $\phi^G_Y(e)$ for its label with respect to its endpoint in $X$ and in $Y$, respectively.
Let $q^t$ be a neighbor query $nbr(v,i)$ where %(without loss of generality)
$v\in X^{t-1}$, \commentt{DR: reminder to add the notation $nbr(\cdot)$ to the preliminaries}
and let $G_{c}$ be a graph in $\calG$ for which the answer to $q^t$ results in a collision. That is,  the answer $a^t$ is $(u,j)$ for some $u\in Y^{t-1}$. 
The neighbors of node $G_{c}$ in $\calG_{nc}$ are nodes representing graphs that can be obtained from $G_{c}$ by swapping the edge $(v,u)$ with a different edge $(v, u')$ where $u'\notin Y^{t-1}$, and  %$G'_{c}$ is consistent with $K^{t-1}$. 
such that the resulting graph belongs to $\calG$.
We prove that there are $\Omega(n^{1/2}\alpha)$ such graphs. 
    
%    The swap modification will maintain the multiplicity of the edge $(v,u)$, and we start describing it for  the case that $(u,v)$ has multiplicity 1.  
In order to modify the graph $G_c \in \calG_c$ to obtain a graph $G_{nc} \in \calG_{nc}$, we proceed as follows.
% Let $\overline{E}^{t-1}(v)$ denote the set of vertex in $Y^{t-1}$
    We choose a vertex \commentt{DR: label?}  $u'\in Y\setminus Y^{t-1}$ (where the constraints on this choice are explained momentarily), and let $v'$ denote the $j$th neighbor of $u'$ in the graph $G_{c}$. Note that $v'$ is in $X$. Let $i'=\phi^{G_c}_X((v',u'))$. Now we swap the pair of  edges $(v,u)$ 
    and $(v',u')$   with the pair  $(v,u'), (v',u)$  while maintaining the original edge-labels. That is, $\phi^{G_{nc}}_X((v,u'))=i, \phi^{G_{nc}}_Y((v,u'))=j$ and $\phi^{G_{nc}}_X((v',u))=i', \phi^{G_{nc}}_Y((v,u'))=j'$. 
    % (Note that this swap might result in multiple edges in the case that either $(v,u')$ or $(v',u)$ are already in  $G'_c$. )
    Since $u' \notin Y^{t-1}$, if $G_{nc}$ is in $\calG$, then it is in $\calG_{nc}$. In order to ensure that $G_{nc}\in\calG$, it is sufficient (and necessary), that there is no edge in $G_c$ between $v$ and $u'$ and no edge between $v'$ and $u$ and that
    $(v',u)\notin \overline{E}^{t-1}$.
    %$v'\notin X^{t-1}$
    %%%%%%%%%%%%%%%%%%%%%%%%%%
    \iffalse
    By the assumption that $u'$ is not in $Y^{t-1}$, 
    and since the degrees of all involved vertices have not changed, and edges were only swapped, 
    it holds that as long as $(v',u)\notin \overline{E}^{t-1}$, the resulting  graph is consistent with $K^{t-1}$. 
    \fi
    %%%%%%%%%%%%%%%%
    
    Observe that the selection of $u'$ uniquely determines $v'$. 
    There are $|Y^{t-1}| \leq t = O(n^{1/4}\alpha^{1/2}$ ``illegal'' choices of $u' \in Y^{t-1}$ and $2\alpha = O(n^{1/4}\alpha^{1/2})$ illegal choices of $u'$ that are neighbors of $v$. There are at most $t$ choices of $v'$ such that $(v',u)\in \overline{E}^{t-1}$, and $d$ choices of neighbors of $u$. For each of these $d+t$ choices of $v'$ there are at most $2\alpha$ neighbors $u'$ such that $v'$ may be the $j$th neighbor of $u'$. This rules out at most $2(d+t)\cdot\alpha$ choices of $u'$.
    Since $|Y|=n\alpha/d$  \commentt{Be precise} and $d = n^{1/2}/c$, for a sufficiently large constant $c$, the number of choices of $u'$ for which $G_{nc} \in \calG$ is $\Omega(n^{1/2}\alpha)$.
    %%%%%%%%%%%%%%%%%%%%%%
    \iffalse
    Since there are $|Y|-|Y^{t-1}|=\Omega(n^{1/2}\alpha)$ options to choose $u'$ (which determines $v'$), and at most $t=O(n^{1/4}\alpha^{1/2})$ of them can result in an edge $(v',u)\in  \overline{E}^{t-1}$, there are $\Omega(n^{1/2}\alpha)$ graphs $G_{nc}$ that are neighbors of $G_{c}$ in $\calB$.
    \fi
    %%%%%%%%%%%%%%%%%%%%

    We now upper bound the number of neighbors of each node  in $\calB$ that corresponds to a graph $G_{nc} \in \calG_{nc}$. 
    Assume that the answer to $q^t=nbr(v,i)$ in $G_{nc}$ is $a^t=(u',j')$. That is, $u'$ is the $i$th neighbor of $v$ in $G_{nc}$, and $v$ is the $j'$th neighbor of $u'$.
      By the definition of $\calB$, every neighbor of $G_{nc}$ in $\calB$ is a graph $G_{c}$ where the $i$th neighbor of $v$ is a vertex $u''\in Y^{t-1}$. Furthermore, by the definition of the swap process, if the edge $(v,u'')\in G_c$ was replaced by a swap process and resulted in an edge $(v,u')$ where $\phi^{G_{nc}}_Y((v,u'))=j'$, it must be the case that $\phi^{G_c}_{Y}((v,u''))=j'$ (since the swapping process  involves only two edges such that both have the same $\phi_Y$ value). Hence, for each choice of $u''\in Y^{t-1}$, the graph $G_c$ from which $G_{nc}$ was obtained by a swap process is uniquely defined: 
      Let $v''$ denote the $j'$th neighbor of $u''$ in $G_c$.
      The graph $G_c$ is a graph where  
      $(v,u'')$ is an edge with $\phi^{G_c}_{X}((v,u''))=i, \phi^{G_c}_Y((v,u''))=j'$ and $(v'', u')$ is an edge with $\phi^{G_c}_Y((v'', u'))=j'$ (and $\phi^{G_c}_X((v'', u'))=i''$ for some $i''$). Since there are at most $|Y^{t-1}|=O(n^{1/4}\alpha^{1/2})$ options to choose $u''$, it holds that $G_{nc}$ has $O(n^{1/4}\alpha^{1/2})$ neighbors in $\calB$ (it might be the case that some of the resulting graphs $G_c$ are not in 
      % the support of $\calD$, 
      $\calG$
      but the upper bound still holds). \commentt{DR: doublecheck superscripts to $\phi$ (and other indices}

 %     Before turning to the general case where there are parallel edges, 
If $q^t = nbr(u,j)$ for $u \in Y^{t-1}$.
 
 Observe that the above argument for the case that $q^t$ is a neighbor query is applicable essentially as is also to the case that $q^t$ is a pair query on a pair of vertices $(u,v)$ (where graphs in $\calG_c$ have an edge between the two vertices and graphs in $\calG_{nc}$ do not).

 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
It remains to address the general  case where graphs in $\calG$ have parallel edges. Once again, consider the case that $q^t$ is a neighbor query on a vertex $v\in X^{t-1}$ (here too the case in which it is a pair query is dealt with essentially the same). Consider any graph $G_c \in \calG_c$ such that  the neighbor query $q^t = (v,i)$  is answered in $\tau(G_c)$ by $(u,j)$ for some $u \in Y^{t-1}$. Denoting by $\ell$ the multiplicity of the edge $(u,v)$ in $G_c$, let $i_1,\dots,i_\ell$ and $j_1,\dots,j_\ell$ be such that for each $r \in [\ell]$, there is an edge $e_r$ in $G_c$ between $u$ and $v$ such that $\phi^{G_c}_X(e_r)=i_r$ and $\phi^{G_c}_Y(e_r)=j_r$.
      In this case all these edges are swapped simultaneously as described next (by generalizing the swap operation for the case when there are no parallel edges).
 %     Let $i=i_1, \ldots, i_l$ be the indices of edges from $v$ to $u$ from the perspective of $v$, and $j=j_1, \ldots, j_{\ell}$ the indices of these edges from the perspective of $u$. To swap the hyper-edge To swap the hyper-edge $(v,u)$, 
 
 We choose a vertex $u'\in Y\setminus Y^{t-1}$  and consider its $j_1,\dots,j_\ell$ incident edges in $G_c$, denoted $e'_1,\dots,e'_\ell$, and the corresponding endpoints, 
$v_1, \ldots, v_{\ell}$ (where these vertices are not necessarily the same nor necessarily distinct). 
 In order to obtain $G_{nc}$ for this choice of $u'$, we first remove the $\ell$ parallel edges between $v$ and $u$ as well as the edges %between $u$ and $v_{j_1},\dots,v_{j_\ell}$. 
 $e'_1,\dots,e'_\ell$ that are incident to $u'$.
 We then  add $\ell$ parallel edges $e_1,\dots,e_\ell$ between $v$ and $u'$
 % an hyper-edge with the  multiplicity  $\ell$ between $v$ to $u'$,
 such that $\phi^{G_{nc}}_X(e_r)= i_r$ and $\phi^{G_{nc}}_Y(e_r)= j_r$ for each $r \in [\ell]$. Finally, we  add edges $e''_1,\dots,e''_\ell$ where $e''_r$ for $r\in [\ell]$ is between $v_{r}$ and $u$, $\phi^{G_{nc}}_X(e''_r) = \phi^{G_c}_X(e'_r)$, and $\phi^{G_{nc}}_Y(e''_r) = j_r$.
 % $(v_{j_1}, u), \ldots, (v_{j_{\ell}}, u)$, such that for every $r\in [1,\ell]$, it holds that  $\phi_X((v_{j_k},u))=\phi_X((u', v_{j_{k}}))$ and $\phi_Y((v_{j_k},u))=j_k$.


  Here too each choice of $u'\in Y\setminus Y^{t-1}$ uniquely determines the vertices $v_1, \ldots v_{\ell}$, and unless $(v_{r},u)\in \overline{E}^{t-1}$, the resulting graph $G_{nc}$ after the swap is consistent with $K^{t-1}$. Hence,  $G_c$ has $\Omega(n^{1/2}\alpha)$ neighbors in $\calB$.
   \commentt{DR: I have to finish from here on, but am a bit unsure about the last statement because of the constraint on non-edges and the possibility of high-multiplicity}
    On the other hand,  consider any graph $G_{nc} \in \calG_{nc}$. 
    For such a graph, the query $q^t = (v,i)$ is answered according to $\tau(G_{nc})$ by $(u',j')$ for $u' \notin Y^{t-1}$.
    Let $e'_1,\dots,e'_{\ell'}$ be the parallel edges between $v$
    and $u'$ in $G_{nc}$ where $\phi^{G_{nc}}_X(e'_r)=i'_r$ and
    $\phi^{G_{nc}}_Y(e'_r)=j'_r$.
    A swap operation on a graph $G_{c} \in \calG_c$ results in $G_{nc}$, only if there exists $u''\in Y^{t-1}$ such that  
    there are $\ell'$ parallel edges $e''_1,\dots,e''_{\ell'}$ between $v$ and $u''$ in $G_c$ where $\phi^{G_C}_Y(e''_r)=j_r$
    %and $\phi^{G_c}_X(e''_r)=i_r$. 
    Therefore, for every  $u''\in Y^{t-1}$, there  is at most  one graph $G_c$ for which the swap operation results in $G_{nc}$, implying that for each $G_{nc}\in \calG_{nc}$, its degree in $\calB$ is $O(n^{1/4}\alpha^{1/2})$. This concludes the proof of the subclaim.
\fi
%%%%%%%%%%%%%%%%%%%
  {\hspace*{\fill}$\Diamond$\par} 
% \end{proof}

\smallskip
By the above, the probability that the algorithm detects a $C_4$ following any one of its at most
$n^{1/4}\alpha^{1/2}/c$ queries is upper bounded by a small constant (e.g., $1/3$).
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{claim}
    Let $q_t$ be a neighbor query $nbr(v,i)$ for some $v\in X$. 
    The number of graphs in the support of $\calD$ that correspond to a collision is smaller by a factor of $\Omega(n^{1/4}\alpha^{1/2})$ than the number of graphs that do not correspond to a collision (henceforth, non-collision graphs).
\end{claim}
\begin{proof}
    We define an  auxiliary bipartite  graphs $\calB$, where each node in $\calB$ corresponds to a graph in the support of $\calD$ that is consistent with $K^{t-1}$.
   Graphs in $\calD$ for which the answer $a^t$ to $q^t$ corresponds to a collision, belong to the left side of $\calB$, denoted $\calB_{c}$, and the others to the right side, denoted $\calB_{nc}$.
    
    
    There is an edge between two nodes in (different sides of) $\calB$, if the graphs they correspond to can be obtained from one another by a ``swap'' modification, which we define below. 
    We shall prove that nodes  on the left side have degree $\Omega(n^{1/2}\alpha)$, while nodes on the right side have degree $O(n^{1/4}\alpha^{1/2})$. Since $\calB$ is bipartite, this implies that $|\calB_{nc}|$ is greater by a factor of $\Omega(n^{1/4}\alpha^{1/2})$ than $\calB_{c}$. By the definition of $\calB$ this will conclude the proof.
    
    Assume first that the query $q^t$ is a neighbor query $(v,i)$, and let $G_{c} \in \calD$ be a graph whose answer to the query results in a collision. That is, assume that the answer $a^t$ is $(u,j)$ for some $u\in K^t$. The neighbors of node $G_{c}$ in $\calB_{nc}$ are nodes that represent graphs that can be obtained from $G_{c}$ by swapping the (hyper-)edge $(v,u)$ in a different (hyper-)edge $(v, u')$ where $u'\notin K^{t-1}$, and  $G'_{c}$ is consistent with $K^{t-1}$. We prove that there are $\Omega(n^{1/2}\alpha)$ such graphs. 
    
    The swap modification will maintain the multiplicity of the edge $(v,u)$, and we start describing it for  the case that $(u,v)$ has multiplicity 1.  In order to modify the graph $G_c$ to get a new graph $G_{nc}$ that is consistent with $K_{t-1}$, we proceed as follows.
    We choose a label  $u'\in Y\setminus V(K_t)$ u.a.r., and let $v'$ denote the $j$th neighbor of $u'$ in the graph $G_{c}$. Note that $v'$ is in $X$. Let $i'$ denote $\phi_X((v',u'))$. Now we swap the pair of  edges $(v,u)$ 
    and $(v',u')$   with the pair  $(v,u'), (v',u)$  while maintaining the original labels. That is, $\phi_X((v,u'))=i, \phi_Y((v,u'))=j$ and $\phi_X((v',u))=i', \phi_Y((v,u'))=j$. 
    % (Note that this swap might result in multiple edges in the case that either $(v,u')$ or $(v',u)$ are already in  $G'_c$. )
    By the assumption that $u'$ is not in $K^{t-1},$ 
    and since the degree of all involved vertices had not changed, and edges were only swapped, 
    it holds that as long as $(v',u)\notin \bar{E}^{t-1}$, the resulting  graph is consistent with $K^{t-1}$. 
    Also, observe that the selection of $u'$ uniquely defines $v'$. 
    Since there are $|Y|-|V(K^{t-1})|=\Omega(n^{1/2}\alpha)$ options to choose $v'$ and at most $t=O(n^{1/4}\alpha^{1/2})$ of them can result in an edge $(v',u)\in  \bar{E}^{t-1}$, there are $\Omega(n^{1/2}\alpha)$ graphs $G_{nc}$ that are neighbors of $G_{c}$ in $\calB$.

    We now upper bound the number of neighbors of each $G_{nc}$ in $\calB$. 
    Assume that the answer to $a_t=nbr(v,i)$ in $G_{nc}$ is $(u',j')$. That is, $u'$ is the $i$th neighbor of $v$ in $G_{nc}$, and $v$ is the $(j')$th neighbor of $u'$.
      By the definition of $\calB$, every neighbor of $G_{nc}$ in $\calB$ is a graph $G_{c}$ where the $i$th neighbor of $v$ is a vertex $u''\in K^{t-1}$. Furthermore, by the definition of the swap process, ifthe edge $(v,u'')\in G_c$ was replaced by a swap process and resulted in edge $(v,u')$ where $\phi_Y((v,u'))=j'$, it must be the case that $\phi_{Y}((v,u''))=j'$ (since the swapping process  involves only two edges such that both have the same $\phi_Y$ value). Hence, for each choice of $u''\in K^{t-1}$, the graph $G_c$ from which $G_{nc}$ was obtained by a swap process is uniquely defined: 
      Let $v''$ denote the $(j')$ neighbor of $u''$ in $G_c$.
      The graph $G_c$ is a graph where  
      $(v,u'')$ is an edge with $\phi_{X}((v,u''))=i, \phi_Y((v,u''))=j'$ and $(v'', u')$ is an edge with $\phi_Y((v'', u'))=j'$ (and $\phi_X((v'', u'))=i''$ for some $i''$). Since there are at most $|V(K^{t-1})|=O(n^{1/4}\alpha^{1/2})$ options to choose $u''$, it holds that $G_{nc}$ has at most $=O(n^{1/4}\alpha^{1/2})$ neighbors in $\calB$ (it might be the case that some of the resulting graphs $G_c$ are not in the support of $\calD$, but the upper bound still holds).

      It remains to address the case where the answer to $a_t$ is an edge $(v,u)$ with multiplicity $\ell>1$. 
      % In this case all the copies of the edge $(v,u)$ are swapped simultaneously as follows. Let $i=i_1, \ldots, i_l$ be the indices of edges from $v$ to $u$ from the perspective of $v$, and $j=j_1, \ldots, j_{\ell}$ the indices of these edges from the perspective of $u$. To swap the hyper-edge  $(v,u)$, we choose a vertex $u'\in Y\setminus K^{t-1}$ u.a.r., and look at its $j_1$ to $j_l$th neighbors,  denoted  $v_{j_1}, \ldots, v_{j_{\ell}}$, respectively. We now remove the hyper-edge $(v,u)$ as well as the edges $(u, v_{j_1}), \ldots, (u,v_{j_{\ell}})$. 
      % % We then  add an hyper-edge with the  multiplicity  $\ell$ between $v$ to $u'$, such that $\phi_Y((v,u'))=\{j_1, \ldots, j_{\ell}\}$, and add edges $(v_{j_1}, u)$
      In this case all the copies of the edge $(v,u)$ are swapped simultaneously as follows. Let $i=i_1, \ldots, i_l$ be the indices of edges from $v$ to $u$ from the perspective of $v$, and $j=j_1, \ldots, j_{\ell}$ the indices of these edges from the perspective of $u$. To swap the hyper-edge To swap the hyper-edge $(v,u)$, we choose a vertex $u'\in Y\setminus V(K^{t-1})$ u.a.r., and look at its $j_1$ to $j_l$th neighbors,  denoted  $v_{j_1}, \ldots, v_{j_{\ell}}$. We now remove the hyper-edge $(v,u)$ as well as the edges $(u, v_{j_1}), \ldots, (u,v_{j_{\ell}})$. We then  add an hyper-edge with the  multiplicity  $\ell$ between $v$ to $u'$, such that $\phi_Y((v,u'))=\{j_1, \ldots, j_{\ell}\}$, and add edges $(v_{j_1}, u), \ldots, (v_{j_{\ell}}, u)$, such that for every $k\in [1,\ell]$, it holds that  $\phi_X((v_{j_k},u))=\phi_X((u', v_{j_{k}}))$ and $\phi_Y((v_{j_k},u))=j_k$.
      Each choice of $u'\in Y\setminus V(K^{t-1})$ uniquely defines the set $v_{j_1}, \ldots v_{j_\ell}$, and unless $(v_{j_k},u)\in \bar{E}^{t-1}$, the resulting graph $G_{nc}$ after the swap is consistent with $K^{t-1}$. Hence,  $G_c$ has $\Omega(n^{1/2}\alpha^{1/4})$ neighbors in $\calB$.
    On the other hand, similarly to what we had before, a graph $G_{c}^*$ can be swapped to $G_{nc}$ above, only if there exists $u''\in V(K^{t-1})$ such that    $(v,u'')$ in $E(G_{c})$ has multiplicity $\ell$ and $\phi_Y((v,u''))=\{j_1, \ldots, j_{\ell}\}$. Therefore, for every  $u''\in V(K^{t-1})$, there  is at most  one graph $G_c^*$ that can be swapped to $G_{nc}$, implying that for each $G_c\in \calB$, its degree in $\calB$ is $O(n^{1/4}\alpha^{1/2})$. This concludes the proof of the subclaim.

%%%%%%%%%%%%
      
%      \commentt{T: I proved the claim on graphs in $\calD$ rather than in $\calD'$ - I'm not sure if that's sufficient}
          

\end{proof}
\fi



\bigskip
Theorem~\ref{thm:C4-gen-alpha-lb} follows by combining Claims~\ref{clm:D-C4-far} and~\ref{clm:D-C4-lb}.
\commentt{DR: or spell it out}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\newpage
\section{From writeup}

\commentt{DR: Base on the following sketch (from the summaries file)}


First we recalled that we have an $\Omega(n^{1/4})$ two-sided error lower bound for constant $\alpha$. I think it is written somewhere, but let's recall quickly. In the FREE instances we have a bipartite graph with $\Theta(n)$ vertices on one side (the left) and $\Theta(n^{1/2})$ on the other. Every vertex on the left has two unique neighbors on the right. In the FAR instances we pair the vertices on the left, and each pair has the same two neighbors on the right. I guess on the right we need to have less vertices, so that we'll also have a small independent set of ``leftover'' vertices. Can consider other (more elegant?) variants, which we may have though of in the past.

Then we recalled the construction for the case that $\alpha = \Theta(n^{1/2})$, for a one-sided error lower bound of $\Omega(n^{1/2})$ (which is $\Omega(n^{1/4} \alpha^{1/2})$). Here (only have FAR instances), on each side we have $\Theta(n)$ vertices with $\Theta(n^{1/2})$ perfect matchings between them. As we noted before, this creates parallel edges, so we need to think whether/how to deal with this. The easy part here is to show the lower bound on the number of queries necessary to see a C4  with constant probability, and the more subtle part (which I think maybe we didn't do in full detail in the past) is showing that whp we indeed get a graph that is far from C4-free. I think in the end (of this meeting) we didn't quite get this to work for $\alpha = \Theta(n^{1/2})$ and constant distance, but only for slightly smaller $\alpha$, and since  both parts of the argument are quite similar for general $\alpha$ (or at least, $\alpha \leq n^{1/2}/\log n$ or so), will turn to that.

The construction for general $\alpha$ still has on one side $\Theta(n)$ vertices (let's say $n$ for simplicity), but on the other side it has $n^{1/2}\alpha$ vertices. The vertices on the lhs have degree $\alpha$, and those on the right have degree $n^{1/2}$.
The edges are selected by picking a random matching between entries of an $n\times \alpha$ table (corresponding to the ``neighbor/edge ports'' of the lhs vertices) and the entries of an $n^{1/2}\alpha \times n^{1/2}$ table (corresponding to the ``neighbor/edge ports of the rhs vertices). Here parallel edges will appear even more, but we continue glossing over this.

To show that $\Omega(n^{1/4} \alpha^{1/2})$ queries are necessary to obtain a C4, we actually show that these many queries are necessary for viewing any cycle. Consider any knowledge graph that is obtained after $n^{1/4} \alpha^{1/2}/c$ queries (for some sufficiently large constant $c$). This graph contains at most $2 n^{1/4} \alpha^{1/2}/c$ vertices. So now, if we condition on this knowledge graph and bound the probability that a neighbor query $(v,i)$ will be answered by some vertex $u$ that is in the knowledge graph, we get that it is at most $2 n^{1/4} \alpha^{1/2}/c$ divided by $n^{1/2}\alpha$, which is $2/(cn^{1/4}\alpha^{1/2})$ (we need to be a bit more precise here -- the conditioning on edges already in the graph only reduces the probability of hitting a vertex in the knowledge graph, but there are also non-edges, and these maybe have an opposite effect). For pair queries it looks like it will be something like $\alpha /(n^{1/2}\alpha) = 1/n^{1/2}$.

Let's turn to showing that we get whp a graph that has $\Omega(m)$ disjoint C4s. The first part of the argument is showing that for every edge, the expected number of C4s that it participates in is $\alpha$.
Consider an edge $(u,v)$. For any choice of sets of neighbors $\Gamma(u)$ and $\Gamma(v)$, and for each pair $(u',v') \in \Gamma(v) \times \Gamma(u)$, the probability that we have an edge between them is (roughly) $\alpha \times 1/(n^{1/2}\alpha) = 1/n^{1/2}$. Since we have $n^{1/2} \cdot \alpha$ such pairs, we get  $\alpha$ in expectation. Hence, for any factor of $2^i$, the fraction of edges that participate in more than $2^i\cdot \alpha$ C4s, is at most $1/2^i$, where the maximum number of C4's that an edge can participate in, is $n^{1/2}\cdot \alpha$. We did a simple bucketing argument, with $O(\log n)$ buckets, by which we got that after removing all edges that reside on more than $c' \alpha$ C4s, we removed at most $\log n \cdot n\alpha \cdot \alpha$ C4s, which for $\alpha$ sufficiently smaller than $(n/\log n)^{1/2}$, is much smaller than $n^2$.

Now we use the fact that the expected number of C4s is $n^4 \cdot (1/n^{1/2})^4 = n^2$. I guess here we need to show that whp we won't get significantly less than this expected value (expectation is not enough, and the C4s are not independent of each other, so maybe need Chebishev).

So we should be left with $\Omega(n^2)$ C4s, where each remaining edge resides on at most $c'\alpha$ (maybe $c'$ is simply $ 2$), so if we run a greedy process for $n\alpha/c''$ iterations, where in each iteration we  assign a ``free'' C4 to an edge (and mark all C4s it participates in as ``un-free''), we'll ``use up'' at most $(n \alpha/c'') \cdot c'\alpha$ C4s, which is less than $(c'/c) n^2$.

Other than doing things more carefully and precisely, there is a question as to whether the $\log n$ factor is really necessary.
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> C4-lb2.tex <==
We begin by describing our construction. For any $n$, $\alpha < n$ and $d> \sqrt{n/\alpha}$, we construct a graph $G = (V, E)$ over $n$ vertices, average degree $d$ and arboricity $\alpha$, such that the following holds.
For any $v\in V$, if we take $q = o()$ length-$2$ random walks from $v$, then with high probability we will not see a $C_4$.
Moreover, $G$ is far from being $C_4$-free. 


\paragraph{The construction}
We shall use the following bipartite graph in one of our lower bounds constructions. 
In this graph, we view one side as corresponding to “lines” and the other to “points”.
So if we view $(a,b)$ as the parameters of a line, then its neighbors are all points $(x,y)$ (in $Z_p \times Z_p$) for which $x = b y  - a$. 

\begin{definition}
[The bipartite graph $G^p_F$]
Let $p$ be a positive integer.
The vertex set of $G^p_F$ is $V_1\cup V_2$ where both in $V_1$ and $V_2$ we have vertices labeled by $Z_p \times Z_p$. There is an edge between $(a,b)\in V_1$ and $(x,y)\in V_2$ iff $x+ a = b\cdot y$ (over $Z_p$). 
\end{definition}

We begin with three disjoint subsets of vertices $V_1$, $V_2$, and $V_3$, each of size $n/3$ (for the sake of brevity we assume that $n$ is divisible by $3$).
We define the following tripartite graph. 
The subgraph induced on $A\cup B$ is $G_F$ (see Definition~\ref{}) where $A$ is one part and $B$ is the other part. Likewise for the subgraph induced on $B\cup C$ w.r.t. $B$ and $C$.
By the construction of $G_F$, at this point for any pair of distinct vertices $u\in B$, $v\in B$, there is a single vertex in $A$ that is adjacent to both vertices and likewise for $C$.
Therefore there is a unique $C_4$ which includes both $u$ and $v$.

We next remove some edges from the graph. For each vertex $v\in B$, with probability $1- p_{\rm ver}$ where $p_{\rm ver} = \alpha/d$, we remove all the edges adjacent to $v$. We then independently remove every edge in the resulting graph with probability $1- p_{\rm e}$ where $p_{\rm e} = d/\sqrt{n}$. This completes the description of the construction. 

\begin{claim}
The graph is far from being $C_4$-free.
\end{claim}
\begin{proof}
    The expected number of $C_4$s is:
    \begin{equation}
        {|V_2| \choose 2} \cdot \left(\frac{\alpha}{d}\right)^2 \left(\frac{d}{\sqrt{n}}\right)^4 = \Theta(\alpha^2 d^2)
    \end{equation}
    Let $(x, y) \in (V_1\times V_2) \cup (V_3\times V_2)$. The expected number of paths of length $3$ from $x$ to $y$ is bounded by 
    \begin{equation}
        \sqrt{n} \cdot p^2_{\rm ver} \cdot p^3_{\rm e} = \theta(\frac{\alpha^2 d}{n}).
    \end{equation} 
\end{proof}
In fact, both hold not only in expectation, but with high probability. This holds by Chebyshev's inequality. To see this, for each pair in $(a, b)\in {V_2 \choose 2}$ consider a random variable $Z_{a,b}$ which is an indicator for the event that there is a $C_4$ which includes both $a$ and $b$ in $G$.
For $a \neq a'$ and $b \neq b'$ it holds that $Z_{a,b}$ and $Z_{a',b'}$ are independent.
Therefore we would like to bound the contribution of $Z_{a,b}$ and $Z_{a,b'}$ to the variance. We have roughly $n^3$ such pairs where each contributes at most $p^3_{\rm ver} \cdot p^6_{\rm e}$. This is divided by $\left(n^2 \cdot p^2_{\rm ver} \cdot p^4_{\rm e}\right)^2$. Hence, the probability to deviate from the expectation by more than a constant factor is at most $1/(n \cdot p_{\rm ver} \cdot p^2_{\rm e}) < 1/(\sqrt{\alpha n})$.
By Chebyshev's inequality, for any non-negative random variable $X$,
\begin{equation}
    \Pr\left[\left|X - E(X)\right| \geq (E(X)/2)\right] \leq \frac{4V(X)}{E^2(X)}
\end{equation}
Taking $X = \sum_{(a, b)\in {V_2 \choose 2}} Z_{a, b}$ and defining $\bar{Z}_{a, b} = Z_{a, b} - \mu$ where $\mu = E_{(a, b)\in {V_2 \choose 2}}[Z_{a, b}]$,  
we obtain that 
\begin{equation}
    \Pr\left[\left|X - E(X)\right| \geq (E(X)/2)\right] \leq \frac{4\sigma_{} E[\bar{Z}_{a, b} \bar{Z}_{a', b'}]}{n^4\mu^2}
\end{equation}

\begin{claim}
Let $v$ be a vertex with $\Gamma_2(v) = s$ and $\ell$ $C_4$s originated from $v$.
If we take $q = $ length-$2$ random walks from $v$, w.h.c.p. we will not see a $C_4$.
\end{claim}

\begin{proof}
Let $S$ denote the set of length-$2$ paths originated from $v$. 
Let $L \subseteq S$ denote the $2\ell$ paths that reside on the $C_4$s originated from $v$.
For the sake of the analysis, we split the process that samples $q$ length-$2$ random walk from $v$ into two steps.
First, it decides for each sample whether it is a walk from $L$ or $S\setminus L$. The former happens with probability $(2\ell)/s$.
After deciding this for each sample, it picks uniformly a random walk from the corresponding set.
Clearly, this is equivalent to selecting uniformly $q$ random walks.

If we pick $q$ random walks, then on expectation, the number of times we pick a random walk from $L$ is $(2\ell q)/s$.
Let $t$ denote this number.
By Chernoff's bound, with high probability, $t$ is concentrated around the expectation. 
Let $E_1$ denote the event that this is indeed the case.

Given $t$, the probability that we don't see a $C_4$ is $(1-1/s)\cdot (1-2/s)\ldots \cdot (1-(t-1)/s) = \Pi_{j=1}^{t-1}\left(1 - j/s\right)$.
Using $(1-1/x)^x \geq 1/e^2$ \commentt{RL: is this a real inequality?} we obtain that this is at least  $\Pi_{j=1}^{t-1} e^{-2j/s} = e^{-t(t-1)/s}$, which is sufficiently large when $t = o(\sqrt{s})$.
The latter happens with high probability when $q = o(s^{3/2}/\ell)$.
\end{proof}

\begin{claim}
    With high probability for every $v\in V$, $s \geq \alpha d$ and $\ell \leq $ 
\end{claim}

==> Ck-ub.tex <==
\section{A general upper bound for $C_k$}\label{sec:Ck}

% \commentt{Change section title? Also order of sections?}

\commentt{I started writing comments in several places. But maybe it is best that I summarize here what are the changes I am planning to make (only in the way things are presented, not in the actual technical details.}

\commentt{
In terms of the order of things, after the definition of $\ell(F)$ (and a short discussion of it), the first algorithm for $F$ (with sampled vertices only) will be presented and analyzed (including the main claim regarding hitting tuples). The corollary for $C_k$ will appear afterwards. Then we shall give the odd-$k$  algorithm for $C_k$, with its analysis (including the edge-sampling).}

\commentt{
I think that the argument regarding the existence of sufficiently many light-vertex-disjoint copies is similar to things we did before, so it can appear in the proofs of the Theorems. 
}

In this we section describe our algorithms for testing 
$C_k$-freeness, for even and odd $k$, and more generally for $F$-freeness. The proofs of correctness follow.
\commentt{maybe use $k$ for $|V(F)|$? Also, do we want to say something here about the running times?}

\newcommand{\VC}{\mathcal{VC}}
\commentt{The problem with the notation $\calC$ is that we used it a lot for a set of edge-disjoint cycles. So maybe $\VC$. Also, using $C$ might not be great, since it might be confused with $C_k$}
\begin{definition}\label{def:ell}
    For a graph $F = (V_F, E_F)$ let $\mathcal{C}(F)$ denote the set of vertex covers of $F$. For a vertex cover $C$ of $F$ we denote by $\mathcal{C'}(C)$ the set of vertex covers of $F$ which are subsets of $C$.
    We define $\ell(F) = max_{C \in \mathcal{C}(F)} \left\{min_{B \in \mathcal{C'}(C)} \left(|B|\right)\right\}$.
\end{definition}
\commentt{Maybe add an explanation about this notion, in particular that it may be much larger than a minimum vertex cover, e.g., for a star?}

\begin{claim}
Let $F = (V_F, E_F)$ and $G = (V_G, E_G)$ be a pair of graphs such that $F$ is a subgraph of $G$. 
Let $C$ be a vertex cover of $G$.
There exists a set of $\ell = \ell(F)$ vertices $v_1, \ldots, v_\ell$ in $C$ such that $E_F \subseteq \bigcup_{i\in [\ell]} \Gamma(v_i)$ where $\Gamma(v)$ denotes the set of edges incident to $v$.  
\commentt{maybe use $E(v)$ because $\Gamma(v)$ is usually used for the neighbors of $v$. Also, I didn't see where we refer to this claim, so I guess it is implicit and maybe we don't need to state it?}
\end{claim}

\begin{proof}
Since $C$ covers the edges of $G$ is also covers the edges of its subgraphs and in particular the edges of $F$. Therefore $D = C\cap V_F$ is a vertex cover of $F$. Consider $B\in \mathcal{C'}(D)$ of minimum size. Such $B$ is a vertex cover of $F$ and its size is at most $\ell(F)$.
Since $B$ is a vertex cover of $F$ it follows that $E_F \subseteq \cup_{v\in B} \Gamma(v)$, as desired.  
\end{proof}


\commentt{shouldn't the algorithms have different names? Or actually, are we keeping only the first one? And if so, are some of the claims later on redundant?}

\commentt{Also, to be consistent with previous parts, I suggest to replace $t$ with $\theta_0$. Also, there is the notion here of light vertices which is only explained later }

\commentt{I wonder how much effort we should put into trying to make things consist with the previous sections}

\commentt{The issue of getting $m$ as input should be discussed somewhere.}

\medskip
    \textsf{Test-$F$-freeness for general $F$}($n, m, \alpha, \epsilon$)  \commentt{Maybe remove ``for general $F$''}
\begin{enumerate}
%\item Obtain $\alpha^*$ (see Claim~\ref{lem:alpha}) and set $t = 48\alpha^*/\epsilon$.
\item Set $t = 4\alpha/\epsilon$.
\item Sample u.a.r. $s = $$\Theta\left(|V(F)|^{2+1/\ell(F)} \cdot m \cdot \left(\frac{\alpha}{m }\right)^{1/\ell(F)} \cdot \left(\frac{1}{\epsilon}\right)^{1+2/\ell(F)}\right)$ vertices (see Definition~\ref{def:ell}).
\item Reveal the neighborhood of all the light vertices (according to $t$) in the sample. 
\item Reject iff there is a witness for $F$ in the resulting subgraph
\end{enumerate}

\medskip
    \textsf{Test-$F$-freeness for general $F$}($n, m, \alpha, \epsilon$)
\begin{enumerate}
%\item Obtain $\alpha^*$ (see Claim~\ref{lem:alpha}) and set $t = 48\alpha^*/\epsilon$.
\item Set $t = 4\alpha/\epsilon$.
\item Sample u.a.r. $h = \Theta\left(|E(F)|^{1+1/|E(F)|} \cdot m^{1-1/|E(F)|} \cdot \left(\frac{1}{\epsilon}\right)^{1/|E(F)|}\right)$ edges from $H(G, t)$ (see Claim~\ref{clm:sample}).
\item Reject iff there is a witness for $F$ in the resulting subgraph
\end{enumerate}


\textsf{Test-$C_k$-freeness when $k$ is odd}($n, m, \alpha, \epsilon$)
\begin{enumerate}
% \item Obtain $\alpha^*$ (see Claim~\ref{lem:alpha}) and set $t = 48\alpha^*/\epsilon$.
\item Set $t = 4\alpha/\epsilon$.
\item Sample u.a.r. $s_1 = \Theta \left(k \cdot m^{1-\frac{2}{k-1}} \cdot (1/\alpha)^{1-\frac{4}{k-1}} \cdot \epsilon^{1-\frac{6}{k-1}}\right)$ edges from the graph. For each edge in the sample,  reveal the neighborhood of both endpoints if both are light. \commentt{I guess this should be the same as in the previous algorithm}
\item If $k > 3$, then sample u.a.r. $s_2 = O\left(k \cdot n \cdot (\alpha^2/m)^{\frac{2}{k-1}} \cdot \left( \frac{1}{\epsilon}\right)^{\frac{6}{k-1}} \right)$ vertices and reveal the neighborhood of all the light vertices in the sample. 
\item Reject iff there is a witness for $F$ in the resulting subgraph.
\end{enumerate}

Before we prove the correctness of the algorithms we shall state several useful definitions and lemmas. 

\commentt{Some of the following is common to all our algorithms. Ideally, I would suggest to  move a general version to the preliminaries and then use it everywhere, or maybe it will be simpler to just say here, the similarly to previous sections, there exists a set $\mathcal{F}$ of at least $\eps m/(2k)$ edge-disjoint copies of $F$ in $G$ (where $k = |V(F)|$ such that no copy includes an edge between two heavy vertices?}

\begin{definition}(\cite{})
For a graph $G = (V, E)$ and a threshold $t$ we define the set of {\em heavy vertices with respect to $t$} as $H_t(G) = \{v\in V: d(v) > t\}$ 
and the set of {\em light vertices with respect to $t$} as $L_t(G) = V \setminus H_t(G)$.
\end{definition}
When $G$ is clear from the context we may simply use $H_t$ and $L_t$. 
Using the definition of $H_t(G)$, we next define the graph $H(G, t)$ which is defined w.r.t. $G$ and a threshold $t$.

\begin{definition}[\bf The undirected graph $H(G, t)$](\cite{})
For a graph $G = (V, E)$ and a threshold $t$, the graph $H(G, t)$ is an undirected graph defined as follows.
The set of vertices of $H(G, t)$ is $V$ and the set of edges of $H(G, t)$ is $E(G)\setminus \{\{u, v\} : u\in H_t(G) \text{ and } v \in H_t(G)\}$.
Namely, $H(G, t)$ is the graph $G$ after removing the edges for which both endpoints are heavy with respect to $t$. 
\end{definition}

\begin{claim}\label{clm:arb}(\cite{})
For a graph $G$, $\alpha' \geq \alpha(G)$ and $\eta\in (0,1]$ it holds that $|E(H(G, \alpha'/\eta))| \geq (1-2\eta)|E(G)|$.
\end{claim}


\begin{claim}\label{lem:alpha}(\cite{})
There exists an algorithm that outputs $\alpha^*$ for which the following holds with probability at least $5/6$:
\begin{enumerate}
\item $|E(H(G, t))| \geq (1-(\eps/6))m$ where $t = 48\alpha^*/\epsilon$,
\item $\alpha^* \leq 2 \alpha(G)$.
\end{enumerate}
\end{claim} 

We say that a pair of subgraphs are {\em light-vertex-disjoint} if they do not share any light vertex (where a light vertex is defined w.r.t. some threshold, depending on the context). 

\begin{claim}\label{clm:disjoint}
Let $G$ be a graph that is $\epsilon$-far from being $F$-free. Let $t$ be a threshold such that $|E(H(G, t))| \geq (1-(\epsilon/2)) |E(G)|$. There exist at least $\epsilon m/ (2t |V(F)|)$ light-vertex-disjoint copies of $F$ in $H(G, t)$ (where a light vertex is defined w.r.t. $t$).
\end{claim}
\begin{proof}
Consider the following process that removes edges from $|E(H(G, t))|$. At each step, if there is a copy of $F$ in the graph, it removes all the edges adjacent to any one of its light vertices. The process terminates after all such edges are removed. Clearly, when the process terminates it has to remove at least $\epsilon m /2$ edges (otherwise we reach a contradiction to the fact that $G$ is $\epsilon$-far from being $F$-free).
At each step, the process removes at most $t \cdot |F|$ edges. Thus, we obtain the desired result. 
\end{proof}

\commentt{What appears below is almost the same as a procedure we already have for sampling edges. But there are some differences. There is also the issue of expected vs maximum}

\medskip
We slightly modify an algorithm from~\cite{} to obtain Claim~\ref{clm:sample}. 

\textsf{Sample a uniform edge from $H(G, t)$}
\begin{enumerate}
\item While do:
\begin{enumerate}
\item Sample u.a.r. a vertex from $V(G)$.
\item Pick $j\in [t]$ and toss a fair coin $b\in \{\rm{Heads}, \rm{Tails}\}$.
\item If $v\in L_t(v)$ and $v$ has a $j$-th neighbour, $u$ then:
\begin{enumerate}
\item If $u \in H_t(G)$ then return $\{u,v\}$. 
\item If $u \in L_t(G)$ and $b=\rm{Heads}$ then return $\{u,v\}$.
\end{enumerate}
\end{enumerate}
\end{enumerate}


\begin{claim}\label{clm:sample}
There exists an algorithm that samples a uniform edge from $H(G, t)$.
If $t$ is such that $|E(H(G, t))| \geq |E(G)|/2$ then the expected running time of the algorithm is $O(t/\bar{d}(G))$. 
\end{claim}



\begin{claim}\label{clm:sampleedges}
Let $S$ be a set of $\beta m$ edges in $H(G, t)$, where $\beta \in (0, 1]$. If we sample $\log n/\beta  \leq y \leq x/2$ edges uniformly from $H(G, t)$, then with high probability we sample at least $c \beta y$ different edges from $x$, where $c$ is an absolute constant. 
\end{claim}

\begin{proof}
    Let $X_i$ denote the indicator variable for the event that the $i$-th sample is an edge from $S$. Since the edges are sampled uniformly from $H(G, t)$, $\Ex(X_i) = \beta$.
    Thus, by multiplicative Chernoff's bound, with high probability $\sum_i X_i = b \beta y$, where $b$ is a constant. 
    Let $Y_i$ be the indicator variable for the event that the $i$-th sample is a new edge from $S$ (with respect the the $(i-1)$ first samples).
    We consider, without loss of generality, the sampling process as if it first decides the values of $X_i$ for each sample $i$ and then sample the edges one by one accordingly.
    Consider the $j$-th sample.
    Given the values of $X_i$ for every $i$ and the values of the samples for each $i < j$, the probability that the $j$-th sample is a new edge, conditioned on the event that $X_j = 1$ is constant (since $y \leq x/2)$. Therefore, with high probability we sample $c \beta y$ different edges from $S$ for some absolute constant $c$. 
\end{proof}

Let $X$ be a set of elements of size $x$ and let $C=\{(v^j_1, \ldots, v^j_\ell)\}_{j\in [|C|]}$ be a set of $\ell$-tuples of elements of $X$ such that each $v\in X$ appears at most once in at most one of the $\ell$-tuples of $C$ (namely, the $\ell$-tuples are disjoint).

Let $S = \{u_1, \ldots u_s\}$ be a set of $s$ elements chosen independently and u.a.r. from $X$. We say that an $\ell$-tuple $(i_1, \ldots i_\ell)$ where $i_j \in s$ for each $j\in [\ell]$ is good w.r.t. $C$ if $(u_{i_1}, \ldots u_{i_\ell})$ belongs to $C$.

We prove the following lemma.

\begin{claim}\label{clm:ver-num}
If $s \geq 16 \ell x / (|C|^{1/\ell})$ then with high constant probability there exists an $\ell$-tuple of $S$ which is good w.r.t. $C$.
\end{claim}

\begin{proof}
Let $\theta$ denote the number of different $\ell$-tuples of $S$.
\commentt{Better not to use $\theta$ for this since we use $\theta_0$ and $\theta_1$ a lot for thresholds. And maybe $\mathcal{L}$ or $\mathcal{T}$ for the tupes?}
Consider all the $\ell$-tuples of $S$ ordered according to some arbitrary order. 
For every $i\in [\theta]$, define $\chi_i$ to be the indicator variable for the event that the $i$-th tuple is good w.r.t. $C$.

\commentt{can we use one of the claims we already have (which we moved from the preliminaries to the appendix) or it doesn't fit?}
We next upper bound the probability that
$\sum_{i \in [\theta]} \chi_{i}=0$.
Let $\bar{\chi}_{i} = \chi_{i} - \mu$, so that $\Ex[\bar{\chi}_{i}] = 0$.
By Chebyshev's inequality,
\begin{equation}\label{eq:cheb-Ck}
\Pr\left[\sum_{i\in [\theta]}\chi_{i}=0\right] \leq \frac{\Var\left[\sum_{i\in [\theta]}\chi_{i}\right]}{\left(\Ex\left[\sum_{i\in [\theta]}\chi_{i}\right]\right)^2}
= \frac{\sum_{i,j} \Ex[\bar{\chi}_{i}\cdot \bar{\chi}_{j}]}{\theta^2\cdot \mu^2} \;.
\end{equation}

We first calculate 
\begin{equation}
\Ex\left[\sum_{i\in [\theta]}\chi_{i}\right] \geq \theta \cdot \mu \geq {s \choose \ell } \cdot \ell! \cdot |C| \cdot \left(\frac{1}{x}\right)^{\ell} 
= \frac{s!}{(s-\ell)!} \cdot |C| \cdot \left(\frac{1}{x}\right)^{\ell} \geq (s/2)^\ell \cdot |C| \cdot \left(\frac{1}{x}\right)^{\ell}  \geq (8\ell)^\ell 
\end{equation}

We next break the sum $\sum_{i,j} \Ex[\bar{\chi}_{i}\cdot \bar{\chi}_{j}]$ into several sub-sums as follows.
We say that $(i,j) \in [\theta]\times [\theta]$ is in $S_t$ if the number of elements (namely, indexes of samples) that belong both to the $i$-th tuple and the $j$-th tuple is exactly $t$ (namely the intersection of the tuples is of size $t$ when they are viewed as sets).  

If $(i,j) \in S_0$ then $\chi_{i}$ and $\chi_{j}$ are independent and so
\begin{equation}\label{eq:cheb-case1}
\Ex[\bar{\chi}_{i}\cdot \bar{\chi}_{j}] =  \Ex[\bar{\chi}_{i}]\cdot \Ex[\bar{\chi}_{j}] = 0\;.
\end{equation}
% where the last iequality follows from the definition of $\bar{\chi}_{i,j}$.
Hence, the pairs in $S_0$ do not contribute anything to the right-hand side of Equation~\eqref{eq:cheb-Ck}.


If $i = j$ then 
\begin{equation}\label{eq:cheb-Ck-case2}
\Ex[\bar{\chi}_{i}\cdot \bar{\chi}_{j}] = \Ex[(\bar{\chi}_{i})^2]
\leq \Ex[(\chi_{i})^2] = \Ex[\chi_{i}] = \mu \;,
\end{equation}
where the second inequality follows from the definition of $\bar{\chi}_{i}$.

Given that $(i,j) \in S_t$ it holds that  

\begin{equation}\label{eq:cheb-Ck-case2}
\Ex[\bar{\chi}_{i}\cdot \bar{\chi}_{j}] 
\leq \Ex[\chi_{i} \chi_{j}] \leq  |C| \cdot \left(\frac{1}{x}\right)^{2\ell -t} \;.
\end{equation}
Since there are at most ${\ell \choose t} \cdot s^{2\ell -t}$ pairs in $S_t$ we obtain that 
\begin{equation}\label{eq:cheb-Ck-case2}
\sum_{(i, j)\in S_t}\Ex[\bar{\chi}_{i}\cdot \bar{\chi}_{j}] 
\leq  {\ell \choose t} \cdot s^{2\ell -t} \cdot |C|\cdot   \left(\frac{1}{x}\right)^{2\ell -t} \leq \ell^t \cdot |C| \cdot \left(\frac{s}{x}\right)^{2\ell -t} \leq  \ell^\ell \cdot |C| \cdot   \left(\frac{s}{x}\right)^\ell =  \left( \frac{|C|^{1/\ell} \cdot \ell \cdot s}{x}\right)^\ell \leq (16\ell^2)^\ell\;,
\end{equation}

Thus,

\begin{equation}
\frac{\sum_{i,j} \Ex[\bar{\chi}_{i}\cdot \bar{\chi}_{j}]}{\theta^2\cdot \mu^2}
\leq  1/(\theta \mu) + (\ell (16\ell^2)^\ell)/(\theta \mu)^2 \leq 
1/ (8\ell)^\ell + (\ell (16\ell^2)^\ell)/(8\ell)^{2\ell} \leq 1/8 + \ell (1/2)^{2\ell} \leq 3/8\;,
\end{equation}
which concludes the proof of the lemma.
\end{proof}

%\begin{equation}\label{eq:cheb-Ck-caseX}
%\Ex[\chi_{i} \chi_{j}] =  \Ex\left[\sum_{h\in [\eta]} \psi^h_{i} \sum_{r \in [\eta]} \psi^r_{j} \right]\;,
%\end{equation}

\begin{theorem}\label{thm:Gen-F-ub}
There exists a one-sided error tester for $F$-freeness whose query complexity is $$O\left(|V(F)|^{2+1/\ell(F)} \cdot m \cdot \left(\frac{\alpha}{m }\right)^{1/\ell(F)} \cdot \left(\frac{1}{\epsilon}\right)^{1+2/\ell(F)}\right)$$ 
\end{theorem}

\begin{proof}
The completeness of the tester follows by construction. 
We next prove its soundness. Assume $G$ is $\epsilon$-far from being $F$-free.
%By Claim~\ref{lem:alpha}, w.p. at least $5/6$,
By Claim~\ref{clm:arb} and the setting of $t$, $|E(H(G, t))| \geq (1-(\epsilon/2)) |E(G)|$. 
Thus, by Claim~\ref{clm:disjoint}, there exist at least $\epsilon m/ (2t |F|)$ light-vertex-disjoint copies of $F$ in $H(G, t)$. \commentt{$|F|$ is $|V(F)|$, right?}
From each one of these copies we pick a subset of light vertices which covers the edges of this copy (since the copy is in $H(G, t)$ there exists a vertex cover which is composed of only light vertices).
Moreover, by the definition of $\ell(F)$, it suffices to pick $\ell(F)$ light vertices for each copy.
By ordering these vertices (arbitrarily) we obtain an $\ell(F)$-tuple of light vertices to each one of these copies.  
Let $C$ to be the set of $\ell(F)$-tuples corresponding to each one of the copies. According to Claim~\ref{clm:ver-num}, if we set $s$ to be at least $16 \ell(F) n / ((\epsilon m/ (2t |F|))^{1/\ell(F)})$ vertices, then w.h.c.p. there exists a copy of $F$ in $G$ such that we hit all its light vertices.
By Claim~\ref{clm:average}, w.h.p., the query complexity of the algorithm is bounded by $s \cdot 2\bar{d} = O\left(|V(F)|^{2+1/\ell(F)} \cdot m \cdot \left(\frac{\alpha}{m }\right)^{1/\ell(F)} \cdot \left(\frac{1}{\epsilon}\right)^{1+2/\ell(F)}\right)$, as desired.
\end{proof}

\begin{corollary}\label{cor:Ck-ub}
There exists a one-sided error tester for $C_k$-freeness whose query complexity is 
$$O\left(k^{2+(2/k))} \cdot m \cdot \left(\frac{\alpha}{m }\right)^{2/k} \cdot \left(\frac{1}{\epsilon}\right)^{1+(4/k)}\right)$$    
for even $k$, and 
$$O\left(k^{2+2/(k+1)} \cdot m \cdot \left(\frac{\alpha}{m }\right)^{2/(k+1)} \cdot \left(\frac{1}{\epsilon}\right)^{1+4/(k+1))}\right)$$    
for odd $k$.
\end{corollary}

The following bound is an improved bound for testing $C_k$-freeness for odd $k$ whenever $m = \Omega(\alpha^{(k+3)/2})$ and in particular when $\alpha$ is a constant.
\begin{theorem}\label{thm:Ck-ub-odd-k}
There exists a one-sided error tester for $C_k$-freeness for odd $k$ whose query complexity is 
$$O\left(k \cdot m \cdot (\alpha^2/m)^{\frac{2}{k-1}} \cdot \left( \frac{1}{\epsilon}\right)^{\frac{6}{k-1}} \right)$$
\end{theorem}

\begin{proof}
The completeness of the tester follows by construction. \commentt{need to say which tester exactly this is}
We next prove its soundness. Assume $G$ is $\epsilon$-far from being $F$-free.
By Claim~\ref{clm:arb} and the setting of $t$, $|E(H(G, t))| \geq (1-(\epsilon/2)) |E(G)|$. 
Thus, by Claim~\ref{clm:disjoint}, there exist at least $\epsilon m/ (2t k)$ light-vertex-disjoint copies of $C_k$ in $H(G, t)$.
From each one of these copies we pick a subset of light vertices which covers the edges of this copy (since the copy is in $H(G, t)$ there exists a vertex cover which is composed of only light vertices).
By the structure of $C_k$, it suffices to pick $\lceil k/2 \rceil$ light vertices from each copy.
Moreover, exactly one pair of these vertices are on the same edge of the corresponding copy $C_k$.
By excluding this pair and ordering the rest of these vertices (arbitrarily) , we obtain an $(k-3)/2)$-tuple of light vertices to each one of these copies.  
Let $X$ denote the set of these tuples.
We also consider the set of pairs of vertices we excluded from each copy.
Each such pair is an edge of a $C_k$. 
Denote this set of edges by $E$.
This set is of size $|X|$ which is at least $\epsilon m/ (2t k)$.
By Claim~\ref{clm:sampleedges}, w.h.p., we sample at least $c \epsilon s_1/ (2t k) $ edges from $E$ (where $c$ is a constant).
Let $C \subseteq X$ be the set of tuples corresponding to copies for which we sampled an edge from $E$.
By the above, w.h.p., $|C| \geq c \epsilon s_1/ (2t k) $. 
Conditioning on this event, according to Claim~\ref{clm:ver-num}, if $s_2$ is at least $16 k n / (c \epsilon s_1/ (2t k))^{2/(k-3)}$, then w.h.c.p. the algorithm will find a copy of $C_k$. 
By Claim~\ref{clm:average} and Claim~\ref{clm:sample}, the expected query complexity of the algorithm is bounded by $O(s_1 \cdot t + s_2 \cdot \bar{d}) = O\left(k \cdot m^{1- \frac{2}{k-1}} \cdot \alpha^{\frac{4}{k-1}} \cdot \left( \frac{1}{\epsilon}\right)^{\frac{6}{k-1}} \right)$, as desired.
\end{proof}

\begin{theorem}\label{thm:Gen-F-ub2}
There exists a one-sided error tester for $F$-freeness whose expected query complexity is $$O\left(|E(F)|^{1+1/|E(F)|} \cdot n\alpha \cdot \left(\frac{1}{m }\right)^{1/|E(F)|} \cdot \left(\frac{1}{\epsilon}\right)^{1+1/|E(F)|}\right)\;.$$ 
\end{theorem}

\begin{proof}
The completeness of the tester follows by construction. 
We next prove its soundness. Assume $G$ is $\epsilon$-far from being $F$-free.
Thus, there exist at least $\epsilon m/ (2|E(F)|)$ edge-disjoint copies of $F$ in $H(G, t)$.
According to Claim~\ref{clm:ver-num}, if we sample at least $16 |E(F)| m / ((\epsilon m/ (2|E(F)|))^{1/|E(F)|})$ edges, then w.h.c.p. there exists a copy of $F$ in $G$ such that we hit all its edges.
The expected query complexity of the algorithm is bounded by $h \cdot (t/\bar{d})$. By the setting of $t$ we obtain the desired result. 
\end{proof}

\input{degrees}

==> degrees.tex <==
\begin{claim}\label{clm:average}
Let $S=\{v_1, \ldots, v_s\}$ be a uniform sample of size at least $s=(t/\bar{d})\cdot 12\ln(1/\delta)$ vertices (with repetitions), where $t$ is any threshold such that $|E(H(G, t))| \geq (1- \epsilon) m$.
Let $\chi_i=d(v_i)$ if $d(v_i)\leq t$ and $\chi_i=0$ otherwise.
Then with probability at least $1-\delta$, $\frac{1}{s}\sum_{i=1}^s\chi_i\leq 2\bar{d}$.
\end{claim}

\begin{proof}
It holds that $\Ex[\chi_i] \leq \frac{1}{n} \sum_{v \in V} d(v) = \bar{d}$.
%Also, let $\mathcal{L}$ denote the set of vertices with degree at most $\alpha/\eps$. In every graph with arboricity at most $\alpha$, there are at most $\eps m$ in the subgraph induced by $V \setminu \mathcal{L}$, and every edge that does not belong to that subgraph has at least one endpoint in $\mathcal{L}$. 
For any $\epsilon < \frac{1}{2}$, 
$\Ex[\chi_i]\geq
\frac{1}{n}\sum_{v \in L_t(G)} d(v) 
\geq \frac{1}{n}\cdot 2(1-\epsilon)m
\geq \bar{d}$.

Also, for every $i\in [s]$, $\chi_i\in [0,t]$ for every $i$. 
Let $x_i=\chi/t$ and $X=\sum_{i=1}^s x_i$.
Then the $x_i$'s are bounded independent   random variables in $[0,1]$ with $\Ex[X]\leq s\cdot \bar{d}/t$. Therefore, by the multiplicative Chernoff's bound
\[
\Pr\left[X > 2s\cdot \frac{\bar{d}}{t}\right] \leq  \Pr[X > 2s\cdot \Ex[X]] < \exp\left( -\frac{\Ex[X]}{3}\right) < \exp\left( -\frac{s\cdot (\bar{d}/4)/(\alpha/\eps)}{3}\right)< \delta.
\]
\end{proof}
